High-throughput Phenotyping of Nematode Cysts

The beet cyst nematode (BCN) Heterodera schachtii is a plant pest responsible for crop loss on a global scale. Here, we introduce a high-throughput system based on computer vision that allows quantifying BCN infestation and characterizing nematode cysts through phenotyping. After recording microscopic images of soil extracts in a standardized setting, an instance segmentation algorithm serves to detect nematode cysts in these samples. Going beyond fast and precise cyst counting, the image-based approach enables quantification of cyst density and phenotyping of morphological features of cysts under different conditions, providing the basis for high-throughput applications in agriculture and plant breeding research.

==> PNS cyst paper/figures.tex <==
\section*{Figures and Tables}

\begin{table}[ht]
\centering
\begin{tabular}{cccccc}
\hline
Data set & Sample name & Sample weight & \# Replicates & \# Images & Description\\
\hline
\multirow{8}{*}{Cyst-Count} & Top-Low-A Debris/Clean & 300g & 6 & 6x(30+12) & \multirow{2}{*}{top soil, low cyst density}\\
& Top-Low-B Debris/Clean & 300g & 6 & 6x(30+12) & \\\cline{2-6}
& Top-High-A Debris/Clean & 300g & 6 & 6x(30+12) & \multirow{2}{*}{top soil, high cyst density}\\
& Top-High-B Debris/Clean & 300g & 6 & 6x(30+12) & \\\cline{2-6}
& Sub-Low-A Debris/Clean & 300g & 6 & 6x(30+12) & \multirow{2}{*}{sub soil, low cyst density}\\
& Sub-Low-B Debris/Clean & 300g & 6 & 6x(30+12) & \\\cline{2-6}
& Sub-High-A Debris/Clean & 300g & 6 & 6x(30+12) & \multirow{2}{*}{sub soil, high cyst density}\\
& Sub-High-B Debris/Clean & 300g & 6 & 6x(30+12) & \\
%\hline
%\multirow{8}{*}{Cyst-Count-Artificial} & OM100-0 & 100g & 8 & 8x30 & \multirow{4}{*}{\shortstack{organic matter from 100g \\ soil sample, mixed with \\ 0, 60, 120, 240 %cysts}}\\
%& OM100-60 & 100g & 8 & 8x30 & \\
%& OM100-120 & 100g & 8 & 8x30 & \\
%& OM100-240 & 100g & 8 & 8x30 & \\\cline{2-6}
%& OM100-0 & 300g & 8 & 8x30 & \multirow{4}{*}{\shortstack{organic matter from 300g \\ soil sample, mixed with \\ 0, 60, 120, 240 cysts}}\\
%& OM100-60 & 300g & 8 & 8x30 & \\
%& OM100-240 & 300g & 8 & 8x30 & \\
%& OM100-120 & 300g & 8 & 8x30 & \\
\hline
\end{tabular}
\caption{Samples used for cyst count validation. The data set contains top soil samples (0-30 cm) and sub soil samples (31-60 cm) of the sugar beet field with different cyst density. Sample A and B were collected after (in March) and before (in September) sugar beet planting period, respectively.}
\label{tab:data}
\end{table}


%Main figures:

\begin{figure}[h]
    \includegraphics[width=\textwidth]{figs/overview.png}
   \caption{Introductory figure: \textbf{a)} Image processing pipeline: a grid of images covering the whole soil sample are processed separately. For each image, patches are processed by the neural network to generate cyst and boundary mask, from which the whole-image masks are stitched and further processed to get the final instance segmentation.  \textbf{b)} Example images containing nematode cysts (annotated in green) and organic debris particles. \textbf{c)} Examples of nematode cysts and debris particles that resemble the cysts.}
	\label{fig:introduction}
\end{figure}

\begin{figure}[h]
   %\includegraphics[width=.6\textwidth]{figs/counts-bar.png}
   %\includegraphics[width=.4\textwidth]{figs/counts-regression.png}
   \includegraphics[width=\textwidth]{figs/count_evaluation.png}
   \caption{Automatic cyst counts are highly correlated with manual cyst counts. \textbf{a)} - \textbf{e)} Manual count, automatic count on a sample with debris and automatic count on a clean sample without debris for different types of soil samples: \textbf{a)} top soil, low cyst density (N = 2 locations * 6 replicates), \textbf{b)} top soil, high cyst density (N = 2*6), \textbf{c)} sub soil, low cyst density (N = 2*6), \textbf{d)} sub soil, high cyst density (N = 2*6). \textbf{e)} Manual count (N = 2*6*4) vs. automatic count on samples with debris and on clean samples. Pearson correlation coefficients for the correlation with manual count results are 0.965 and 0.987, respectively. %Both automatic count results can be fitted by linear regression model: The y offset is higher for the debris samples, indicating a slight, but consistent, overcounting of cysts due to debris particles that resemble cysts.
   }
	\label{fig:cyst_count_manual}
\end{figure}

%\begin{figure}[h]
%    \includegraphics[width=.5\textwidth]{figs/counts-art-bar.png}
%    \caption{Cyst count validation: Artificial data with hand-picked cysts}
%	\label{fig:cyst_count_artificial}
%\end{figure}

\begin{figure}[h]
    \centering
    %\includegraphics[width=.5\textwidth]{figs/PPV_FNR_curve.png}\hfill
	%\includegraphics[width=.5\textwidth]{figs/scores.png}\\
	%\includegraphics[width=.5\textwidth]{figs/seg_demo1.png}
	\includegraphics[width=\textwidth]{figs/seg_evaluation.png}
   \caption{Cyst segmentation validation. \textbf{a)} PPR and FNR achieved by the computer vision pipeline (with ResNet 101 backbone) over a range of IoU thresholds. For comparison, we include three further network architecures (ResNet 50, 152, U-Net). \textbf{b)} Segmentation quality measures (Methods) for the computer vision pipeline with ResNet 101 and for the architectural variants. \textbf{c)} Qualitative examples for cyst segmentation masks obtained with the computer vision pipeline. Red lines indicate the ground truth boundary. Some instance masks are annotated with IoU scores.}
	\label{fig:segmentation}
\end{figure}


\begin{figure}[h]
    \centering
    \includegraphics[width= 0.5\textwidth]{figs/cyst_size_seg.pdf}
    \includegraphics[width= 0.5\textwidth, page=2]{figs/cyst_size.pdf}
    \caption{Characterizing nematode cysts by cyst size (area in pixels) as a phenotypical feature.
    \textbf{a)} Cyst size estimates based on automatic segmentation are similar to those based on manually annotated cysts. On the \emph{Cyst\_segmentation} data (with debris), $1366$ (automatic) and $1399$ (manual) cysts, respectively, were detected and segmented. Density functions show the relative proportion of cysts of a certain size (x axis) for the respective distribution. The means of the distributions (automatic: $2164.86$, manual: $2226.71$) are marked by dashed lines.
    \textbf{b)} Characterizing two nematode populations in terms of cyst size. On the \emph{Cyst\_count} data (Table~\ref{tab:data}, clean samples without debris), $4503$ cysts were detected by the automatic method in top soil (0-30 cm) and $2714$ in sub soil (31-60 cm). Density functions visualize the relative proportion of cysts of a certain size. The means of the distributions (top soil: $2732.48$, sub soil: $2913.09$) are marked by dashed lines.
}
\label{fig:phenotyping}
\end{figure}



%Supplementary figures
\beginsupplement

%\begin{figure}[h]
%   \caption{Examples for mistakes: FPs, missed cysts, cysts not separated}
%	\label{fig:error_analysis}
%\end{figure}

%\begin{figure}[h]
%   \caption{Example images from the artificial data}
%	\label{fig:artificial_data}
%\end{figure}

\begin{figure}[h]
    \begin{center}
    \includegraphics[width=.5\textwidth]{figs/image_recording.png}
    \caption{Microscopical image recording setup LemnaTec PhenoAIpert HM (High Magnification).}
	\label{fig:image_recording}
	\end{center}
\end{figure}



